WaveCorr: Correlation-savvy Deep Reinforcement Learning for Portfolio Management

The problem of portfolio management represents an important and challenging class of dynamic decision making problems, where rebalancing decisions need to be made over time with the consideration of many factors such as investors preferences, trading environments, and market conditions. In this paper, we present a new portfolio policy network architecture for deep reinforcement learning (DRL)that can exploit more effectively cross-asset dependency information and achieve better performance than state-of-the-art architectures. In particular, we introduce a new property, referred to as \textit{asset permutation invariance}, for portfolio policy networks that exploit multi-asset time series data, and design the first portfolio policy network, named WaveCorr, that preserves this invariance property when treating asset correlation information. At the core of our design is an innovative permutation invariant correlation processing layer. An extensive set of experiments are conducted using data from both Canadian (TSX) and American stock markets (S&P 500), and WaveCorr consistently outperforms other architectures with an impressive 3%-25% absolute improvement in terms of average annual return, and up to more than 200% relative improvement in average Sharpe ratio. We also measured an improvement of a factor of up to 5 in the stability of performance under random choices of initial asset ordering and weights. The stability of the network has been found as particularly valuable by our industrial partner.

==> WaveCorr NeurIPS/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> WaveCorr NeurIPS/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> WaveCorr NeurIPS/oldTex/oldMDP.tex <==
\subsection{Risk-averse Reinforcement Learning Formulation}\label{sec:RL}

In this section, we formulate the potfolio management problem as a Markov Decision Process (MDP) denoted by $(\mathcal{S},\mathcal{A},\mathcal{T},r)$. In this regard, the agent (i.e. an investor) interacts with a stochastic environment by taking an action $a_t \equiv \PW_t\in \mathbb{W}$ after observing the state $s_t \in \mathcal{S}$ composed of a window of historical market observations, which include the latest stock returns $\Areturns_{t}$, along with the final portfolio composition of the previous period $\PW_t'$. This action results in the immediate stochastic reward that takes the shape of an approximation of the realized log return, i.e. $r_{t+1}(s_t,a_t) := \ln(f(1,\PW_t',\PW_t))+\ln(\Areturns_{t+1}^T \PW_t)\approx\ln(\nu(\PW_t',\PW_t))+\ln(\Areturns_{t+1}^T \PW_t) $, for which a derivative is easily obtained.  
%In the literature two different approaches exist for choosing the actions in each state of an RL model, stochastic and deterministic. However, as mentioned by \cite{silver2014deterministic} stochastic policies require more samples for training compared to deterministic policies. Since we work with real market data and not synthetic data sets, we choose to follow deterministic policies. 
Finally, $\mathcal{T}$ captures the assumed Markovian transition dynamics of the stock market and its effect on portfolio weights: $P(s_{t+1}|s_0,a_0,s_1,a_1,...,s_t,a_t)=\mathcal{T}(s_{t+1}|s_t,a_t)$. 
%By sequentially interacting with the environment, the agent creates trajectories of states, actions, and rewards, $s_0,a_0,r_0,...,s_T,a_T,r_T$ in the space of $\mathcal{S} \times \mathcal{A} \times \mathcal{R}$. 

%The goal is then to maximize a function of the future rewards starting from an initial state $s_0$:
%\begin{equation}\nonumber
%\begin{aligned}
%&\max_\mu f(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1}))\\
%&s.t.\\
%&s_{t+1} \sim \mathcal{T}(s_{t+1}|s_t,a_t),\\
%&a_t=\mu(s_t)
%\end{aligned}
%\end{equation}

% Following the works of \cite{moody2001learning,almahdi2017adaptive}, we choose the function $f$ to be the expected value of the Sharpe ratio over the sequential log-returns of the portfolio:
% \begin{equation}
% \begin{aligned}
% f(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1})) &= \mathbb{E}(SR(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1})))\\
% SR(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1})) &= \frac{Average(r_t)}{Standard Deviation(r_t)} = \frac{A_T}{\sqrt{\frac{T}{T-1}(B_T-A_T)}}\\
% A_T&=\frac{1}{T}\sum_{t=1}^T r_t, \quad B_T = \frac{1}{T}\sum_{t=1}^T r^2_t
% \end{aligned}
% \end{equation}

Following the works of \cite{moody1998performance,almahdi2017adaptive} on risk averse DRL, our objective is to identify a deterministic trading policy $\mu_\theta$ (parameterized by $\theta$) that maximizes the expected value of the Sharpe ratio measured on $T$-periods log-return trajectories generated by $\mu_\theta$. Namely:
\begin{eqnarray} \label{mainprob}
\max_
\theta\quad J_F(\mu_\theta):=\mathbb{E}_{s_0\sim F,s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\mu_\theta(s_t))}[SR(r_1(s_0,\mu_\theta(s_0)),...,r_T(s_{T-1},\mu_\theta(s_{T-1})))]
\end{eqnarray}
where $F$ is some fixed distribution and
\begin{equation}
\begin{aligned}
SR(r_{1:T}) &:= \frac{(1/T)\sum_{t=1}^T r_t}{\sqrt{(1/(T-1))\sum_{t=1}^T (r_t-(1/T)\sum_{t=1}^T r_t)^2}}\,.
\end{aligned}
\end{equation}
The choice of using the Sharpe ratio of log returns is motivated by modern portfolio theory (see \cite{markowitz1959portfolio}) which advocates a balance between expected returns and exposure to risks, and where it plays the role of a canonical way of exercising this trade-off \citep{sharpeRatio}. While it is inapt of characterizing downside risk, it is still considered ``gold standard of performance evaluation" by the financial community \citep{bailey2012sharpe}. In \cite{moody1998performance}, the trajectory-wise Sharpe ratio is used as an estimator of the instantaneous one in order to facility its use in RL. A side-benefit of this estimator is to offer some control on the variations in the evolution of the portfolio value which can be reassuring for the investor.



In the context of our portfolio management problem, since $s_t$ is composed of an exogeneous component $s_t^{exo}$ which includes $\Areturns_{t-1}$ and an endogenous state $\PW_t'$ that becomes deterministic when $a_t$ and $s_{t+1}^{exo}$ are known, we have that:
%\[J_F(\mu_\theta):=\mathbb{E}_{\substack{s_0\sim F\\s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}}[SR(\preturn_1(\mu_\theta(\bar{s}_0(s_0,\mu_\theta)),\Areturns_1),\dots,\preturn_T(\mu_\theta(\bar{s}_{T-1}(s_{0:T-1},\mu_\theta)),\Areturns_T))]\] 
%\[J_F(\mu_\theta):=\mathbb{E}_{\substack{s_0\sim F\\s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}}[SR(r_1(\bar{s}_0(s_0,\mu_\theta),\mu_\theta(\bar{s}_0(s_0,\mu_\theta))),\dots,r_T(\bar{s}_{T-1}(s_{0:T-1},\mu_\theta),\mu_\theta(\bar{s}_{T-1}(s_{0:T-1},\mu_\theta))))]\]
\[J_F(\mu_\theta):=\mathbb{E}_{\substack{s_0\sim F\\s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}}[SR(r_1(\bar{s}_0^\theta,\mu_\theta(\bar{s}_0^\theta))
,\dots,r_T(\bar{s}_{T-1}^\theta,\mu_\theta(\bar{s}_{T-1}^\theta)))]\]
where $\beta(s_t)$ is an arbitrary policy, and where the effect of $
\mu_\theta$ on the trajectory can be calculated using 
%\[\bar{s}_t(s_{0:t},\mu_\theta):=\left(s_{t}^{exo},\frac{\Areturns_{t}\circ\mu_\theta(\bar{s}_{t-1}(s_{0:t-1},\mu_\theta))}{\Areturns_{t+1}^T \mu_\theta(\bar{s}_{t-1}(s_{0:t-1},\mu_\theta))}\right)\,,\]
\[\bar{s}_t^\theta:=\left(s_{t}^{exo},\frac{\Areturns_{t}\circ\mu_\theta(\bar{s}_{t-1}^\theta)}{\Areturns_{t}^T \mu_\theta(\bar{s}_{t-1}^\theta)}\right)\,,\]
for $t\geq 1$, %and $\bar{s}_1(s_{0},\mu_\theta):=(s_1^{exo},\mu_\theta(s_0))$ 
while $\bar{s}_0^\theta:=s_0$. %$\bar{s}_0(s_0,\mu_\theta):=s_0$.
Hence,
%\[\nabla_\theta J_F(\mu_\theta):=\mathbb{E}%_{s_0\sim F,s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}
%%[\nabla_\theta SR(\preturn_1(\mu_\theta(\bar{s}_0(s_0,\mu_\theta)),\Areturns_1),
%\dots,\bar{r}_T^p(\mu_\theta(\bar{s}_{T-1}(s_{0:t-1},\mu_\theta)),\bar{r}_T))]\,,\]
\[\nabla_\theta J_F(\mu_\theta):=\mathbb{E}%_{s_0\sim F,s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}
[\nabla_\theta SR(r_1(\bar{s}_0^\theta,\mu_\theta(\bar{s}_0^\theta)),
\dots,r_T(\bar{s}_{T-1}^\theta,\mu_\theta(\bar{s}_{T-1}^\theta)))]\,,\]
where $\nabla_\theta SR$ can be obtained by backpropagation using the chain rule. This leads to the following stochastic gradient step:
%\[    \theta_{k+1} = \theta_k + \alpha \nabla_\theta SR(\bar{r}_1^p(\mu_\theta(\bar{s}_0(s_0,\mu_\theta)),\bar{r}_1), \dots,\bar{r}_T^p(\mu_\theta(\bar{s}_{T-1}(s_{0:t-1},\mu_\theta)),\bar{r}_T))\,,\]
\[    \theta_{k+1} = \theta_k + \alpha \nabla_\theta SR(r_1(\bar{s}_0^\theta,\mu_\theta(\bar{s}_0^\theta)), \dots,r_T(\bar{s}_{T-1}^\theta,\mu_\theta(\bar{s}_{T-1}^\theta))\,,\]
with $\alpha>0$ as the step size.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> oldTex/oldMDP.tex <==
\subsection{Risk-averse Reinforcement Learning Formulation}\label{sec:RL}

In this section, we formulate the potfolio management problem as a Markov Decision Process (MDP) denoted by $(\mathcal{S},\mathcal{A},\mathcal{T},r)$. In this regard, the agent (i.e. an investor) interacts with a stochastic environment by taking an action $a_t \equiv \PW_t\in \mathbb{W}$ after observing the state $s_t \in \mathcal{S}$ composed of a window of historical market observations, which include the latest stock returns $\Areturns_{t}$, along with the final portfolio composition of the previous period $\PW_t'$. This action results in the immediate stochastic reward that takes the shape of an approximation of the realized log return, i.e. $r_{t+1}(s_t,a_t) := \ln(f(1,\PW_t',\PW_t))+\ln(\Areturns_{t+1}^T \PW_t)\approx\ln(\nu(\PW_t',\PW_t))+\ln(\Areturns_{t+1}^T \PW_t) $, for which a derivative is easily obtained.  
%In the literature two different approaches exist for choosing the actions in each state of an RL model, stochastic and deterministic. However, as mentioned by \cite{silver2014deterministic} stochastic policies require more samples for training compared to deterministic policies. Since we work with real market data and not synthetic data sets, we choose to follow deterministic policies. 
Finally, $\mathcal{T}$ captures the assumed Markovian transition dynamics of the stock market and its effect on portfolio weights: $P(s_{t+1}|s_0,a_0,s_1,a_1,...,s_t,a_t)=\mathcal{T}(s_{t+1}|s_t,a_t)$. 
%By sequentially interacting with the environment, the agent creates trajectories of states, actions, and rewards, $s_0,a_0,r_0,...,s_T,a_T,r_T$ in the space of $\mathcal{S} \times \mathcal{A} \times \mathcal{R}$. 

%The goal is then to maximize a function of the future rewards starting from an initial state $s_0$:
%\begin{equation}\nonumber
%\begin{aligned}
%&\max_\mu f(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1}))\\
%&s.t.\\
%&s_{t+1} \sim \mathcal{T}(s_{t+1}|s_t,a_t),\\
%&a_t=\mu(s_t)
%\end{aligned}
%\end{equation}

% Following the works of \cite{moody2001learning,almahdi2017adaptive}, we choose the function $f$ to be the expected value of the Sharpe ratio over the sequential log-returns of the portfolio:
% \begin{equation}
% \begin{aligned}
% f(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1})) &= \mathbb{E}(SR(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1})))\\
% SR(r_1(s_0,a_0),...,r_T(s_{T-1},a_{T-1})) &= \frac{Average(r_t)}{Standard Deviation(r_t)} = \frac{A_T}{\sqrt{\frac{T}{T-1}(B_T-A_T)}}\\
% A_T&=\frac{1}{T}\sum_{t=1}^T r_t, \quad B_T = \frac{1}{T}\sum_{t=1}^T r^2_t
% \end{aligned}
% \end{equation}

Following the works of \cite{moody1998performance,almahdi2017adaptive} on risk averse DRL, our objective is to identify a deterministic trading policy $\mu_\theta$ (parameterized by $\theta$) that maximizes the expected value of the Sharpe ratio measured on $T$-periods log-return trajectories generated by $\mu_\theta$. Namely:
\begin{eqnarray} \label{mainprob}
\max_
\theta\quad J_F(\mu_\theta):=\mathbb{E}_{s_0\sim F,s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\mu_\theta(s_t))}[SR(r_1(s_0,\mu_\theta(s_0)),...,r_T(s_{T-1},\mu_\theta(s_{T-1})))]
\end{eqnarray}
where $F$ is some fixed distribution and
\begin{equation}
\begin{aligned}
SR(r_{1:T}) &:= \frac{(1/T)\sum_{t=1}^T r_t}{\sqrt{(1/(T-1))\sum_{t=1}^T (r_t-(1/T)\sum_{t=1}^T r_t)^2}}\,.
\end{aligned}
\end{equation}
The choice of using the Sharpe ratio of log returns is motivated by modern portfolio theory (see \cite{markowitz1959portfolio}) which advocates a balance between expected returns and exposure to risks, and where it plays the role of a canonical way of exercising this trade-off \citep{sharpeRatio}. While it is inapt of characterizing downside risk, it is still considered ``gold standard of performance evaluation" by the financial community \citep{bailey2012sharpe}. In \cite{moody1998performance}, the trajectory-wise Sharpe ratio is used as an estimator of the instantaneous one in order to facility its use in RL. A side-benefit of this estimator is to offer some control on the variations in the evolution of the portfolio value which can be reassuring for the investor.



In the context of our portfolio management problem, since $s_t$ is composed of an exogeneous component $s_t^{exo}$ which includes $\Areturns_{t-1}$ and an endogenous state $\PW_t'$ that becomes deterministic when $a_t$ and $s_{t+1}^{exo}$ are known, we have that:
%\[J_F(\mu_\theta):=\mathbb{E}_{\substack{s_0\sim F\\s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}}[SR(\preturn_1(\mu_\theta(\bar{s}_0(s_0,\mu_\theta)),\Areturns_1),\dots,\preturn_T(\mu_\theta(\bar{s}_{T-1}(s_{0:T-1},\mu_\theta)),\Areturns_T))]\] 
%\[J_F(\mu_\theta):=\mathbb{E}_{\substack{s_0\sim F\\s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}}[SR(r_1(\bar{s}_0(s_0,\mu_\theta),\mu_\theta(\bar{s}_0(s_0,\mu_\theta))),\dots,r_T(\bar{s}_{T-1}(s_{0:T-1},\mu_\theta),\mu_\theta(\bar{s}_{T-1}(s_{0:T-1},\mu_\theta))))]\]
\[J_F(\mu_\theta):=\mathbb{E}_{\substack{s_0\sim F\\s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}}[SR(r_1(\bar{s}_0^\theta,\mu_\theta(\bar{s}_0^\theta))
,\dots,r_T(\bar{s}_{T-1}^\theta,\mu_\theta(\bar{s}_{T-1}^\theta)))]\]
where $\beta(s_t)$ is an arbitrary policy, and where the effect of $
\mu_\theta$ on the trajectory can be calculated using 
%\[\bar{s}_t(s_{0:t},\mu_\theta):=\left(s_{t}^{exo},\frac{\Areturns_{t}\circ\mu_\theta(\bar{s}_{t-1}(s_{0:t-1},\mu_\theta))}{\Areturns_{t+1}^T \mu_\theta(\bar{s}_{t-1}(s_{0:t-1},\mu_\theta))}\right)\,,\]
\[\bar{s}_t^\theta:=\left(s_{t}^{exo},\frac{\Areturns_{t}\circ\mu_\theta(\bar{s}_{t-1}^\theta)}{\Areturns_{t}^T \mu_\theta(\bar{s}_{t-1}^\theta)}\right)\,,\]
for $t\geq 1$, %and $\bar{s}_1(s_{0},\mu_\theta):=(s_1^{exo},\mu_\theta(s_0))$ 
while $\bar{s}_0^\theta:=s_0$. %$\bar{s}_0(s_0,\mu_\theta):=s_0$.
Hence,
%\[\nabla_\theta J_F(\mu_\theta):=\mathbb{E}%_{s_0\sim F,s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}
%%[\nabla_\theta SR(\preturn_1(\mu_\theta(\bar{s}_0(s_0,\mu_\theta)),\Areturns_1),
%\dots,\bar{r}_T^p(\mu_\theta(\bar{s}_{T-1}(s_{0:t-1},\mu_\theta)),\bar{r}_T))]\,,\]
\[\nabla_\theta J_F(\mu_\theta):=\mathbb{E}%_{s_0\sim F,s_{t+1}\sim\mathcal{T}(s_{t+1}|s_t,\beta(s_t)))}
[\nabla_\theta SR(r_1(\bar{s}_0^\theta,\mu_\theta(\bar{s}_0^\theta)),
\dots,r_T(\bar{s}_{T-1}^\theta,\mu_\theta(\bar{s}_{T-1}^\theta)))]\,,\]
where $\nabla_\theta SR$ can be obtained by backpropagation using the chain rule. This leads to the following stochastic gradient step:
%\[    \theta_{k+1} = \theta_k + \alpha \nabla_\theta SR(\bar{r}_1^p(\mu_\theta(\bar{s}_0(s_0,\mu_\theta)),\bar{r}_1), \dots,\bar{r}_T^p(\mu_\theta(\bar{s}_{T-1}(s_{0:t-1},\mu_\theta)),\bar{r}_T))\,,\]
\[    \theta_{k+1} = \theta_k + \alpha \nabla_\theta SR(r_1(\bar{s}_0^\theta,\mu_\theta(\bar{s}_0^\theta)), \dots,r_T(\bar{s}_{T-1}^\theta,\mu_\theta(\bar{s}_{T-1}^\theta))\,,\]
with $\alpha>0$ as the step size.
